Leveraging Medical Visual Question Answering with Supporting Facts

In this working notes paper, we describe IBM Research AI (Almaden) team's participation in the ImageCLEF 2019 VQA-Med competition. The challenge consists of four question-answering tasks based on radiology images. The diversity of imaging modalities, organs and disease types combined with a small imbalanced training set made this a highly complex problem. To overcome these difficulties, we implemented a modular pipeline architecture that utilized transfer learning and multi-task learning. Our findings led to the development of a novel model called Supporting Facts Network (SFN). The main idea behind SFN is to cross-utilize information from upstream tasks to improve the accuracy on harder downstream ones. This approach significantly improved the scores achieved in the validation set (18 point improvement in F-1 score). Finally, we submitted four runs to the competition and were ranked seventh.

==> dataset.tex <==
\section{Brief Analysis of the VQA-Med dataset}
\label{sec:dataset}

The VQA-Med dataset~\cite{ImageCLEFVQA-Med2019} is a new VQA dataset embedded in the medical domain, with a focus on radiology images. More details about the dataset can be found in ~\cite{ImageCLEFVQA-Med2019}.  Here, we will briefly describe the tasks and summarize our analysis, which was crucial in developing the  solution presented in this work. 

The dataset consists of the following three splits:
\begin{itemize}
\item a training set of 3,200 images with 12,792 Question-Answer (QA) pairs,
\item a validation set of 500 images with 2,000 QA pairs, and
\item a test set of 500 images with 500 questions (\rs\ answers were released after the end of the VQA-Med 2019 challenge).
\end{itemize}
In all splits the samples were divided into four categories, depending on the main task to be solved:
\begin{itemize}
\item \CM: determine the modality of the image, 
\item \CP: determine the plane of the image,
\item \CO: identify the organ/anatomy of interest in the image, and
\item \CA: identify the abnormality in the image. 
\end{itemize}

% Training set categories (1292): C1	2016		C2	3200	C3	3200	C4	3082	BINARY		1294
% Validation set categories (2000): C1	321	C2	500	C3	500	C4	477	BINARY		202
% Test set categories (500): 	C1		72		C2	125	C3	125	C4	114	BINARY		64

In the first step we have analyzed the types and distributions of questions in all four categories (\Fig{question_distributions}).
Our first observation was the simplicity of the questions with a small vocabulary (98 different words) and the lack a compositional structure.
Second, the question types for each category are very distinctive. Thus, we hypothesized that the task category can be determined by pure analysis of the question and the problem can be solved with four specialized image classifiers.
However, as some questions contain some \textit{keywords} that might be used as additional cues during reasoning (e.g. "is this image modality \textit{t1}, \textit{t2} or \textit{flair}?") we decided that our models should use question/text modality as an additional input.

\begin{figure}[h!]
\subfloat[\CM: Modality]{%
	\includegraphics[width=0.5\textwidth]{distributions/c1_training_set_questions.png}
}
\subfloat[\CP: Plane]{%
	\includegraphics[width=0.5\textwidth]{distributions/c2_training_set_questions.png}
}
\\
\subfloat[\CO: Organ]{%
	\includegraphics[width=0.5\textwidth]{distributions/c3_training_set_questions.png}
}
\subfloat[\CA: Abnormality]{%
	\includegraphics[width=0.5\textwidth]{distributions/c4_training_set_questions.png}
}
\caption{Distribution of questions in the original four categories.}
\label{fig:question_distributions}
\end{figure}

Next we analyzed the provided ground-truth answers (\Fig{answers_distributions}), which showed that category distributions are extremely imbalanced, sometimes with a single answer being heavily over-represented (e.g. \textit{axial} in \CP or \textit{skull and contents} in \CO).
This observation led us to use weighted sampling.

Besides, we have noticed that in \CM and \CA two most frequent answers were \textit{Yes} and \textit{No}, which indicates the presence of a significant number of binary questions.
Therefore, we decided to distinguish a fifth category, \CB, and this reinforced our decision to incorporate a specialized module to determine the question category.
\Fig{question_categories} shows the resulting distributions of question categories, where questions with answers belonging to \CB account for 10\% percent of the training data.

\begin{figure}[t!]
\subfloat[\CM: Modality]{%
	\includegraphics[height=2.4cm]{distributions/c1_training_set_answers.png}
}
\subfloat[\CP: Plane]{%
	\includegraphics[height=2.4cm]{distributions/c2_training_set_answers.png}
}
\subfloat[\CO: Organ]{%
	\includegraphics[height=2.4cm]{distributions/c3_training_set_answers.png}
}\\
\subfloat[\CA: Abnormality]{%
	\includegraphics[width=\textwidth]{distributions/c4_training_set_answers.png}
}
\caption{Distribution of answers in the original four categories.}
\label{fig:answers_distributions}
\end{figure}

After closer analysis of different classes of answers we saw that some answer classes could be merged. 
For example, three classes in \CM:
\begin{itemize}
\item \textit{ct - gi \& iv contrast},
\item \textit{ct with gi and iv contrast},
\item \textit{gi and iv}
\end{itemize}
refer to exactly the same computed tomography contrast scan.
Please notice that the first two classes could be merged automatically using standard NLP pre-processing techniques (removing punctuation and stop words).
However, as the main metric used in the challenge was \textit{strict accuracy} we decided to skip data cleaning as it could potentially degrade the final score (still leaving 33\% change of hitting the right answer though).

\begin{figure}[b!]
\centering
%\includegraphics[width=0.5\textwidth]{test_set_queestion_categories.png}
\subfloat[Training set]{%
	\includegraphics[height=2.55cm]{distributions/training_set_question_categories.png}
}
\subfloat[Validation set]{%
	\includegraphics[height=2.55cm]{distributions/validation_set_question_categories.png}
}
\subfloat[Test set\rs]{%
	\includegraphics[height=2.55cm]{distributions/test_set_question_categories_predicted.png}
}
\caption{Distributions of question categories in different sets after introduction of the fifth \CB (Yes/No) category (\rs distribution predicted by \textbf{Question Categorizer}).}
\label{fig:question_categories}
\end{figure}


\begin{table}[t!]
	\begin{center}
		\begin{tabular}{c@{\extracolsep{5pt}}c@{\extracolsep{5pt}}c@{\extracolsep{5pt}}c@{\extracolsep{5pt}}c}
			\toprule
			Category & Training  & Validation New & Training + Validation & Test New\rs  \\
			\cmidrule{1-1} \cmidrule{2-2}  \cmidrule{3-3}  \cmidrule{4-4} \cmidrule{5-5}
			\CM & 42 & 1 & 43 & 2 \\
			\CP & 15 & 1 & 16 & 0 \\
			\CO &  10 &  0 & 10 &  0 \\
			\CA & 1483 & 147 & 1630 & 41 \\
			\CB & 2 & - & - & - \\
			\midrule
			Total & 1550 & 149 & 1699 & 43 \\
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{Number of unique answer classes per category (\rs  indicates new classes found in the Test Set answers released after the end of the VQA-Med 2019 challenge).}
	\label{tab:answers_statistics}
\end{table}

Next we have analyzed the validation set.
Surprisingly, we found that the validation set contains answers that were not present in the training set -- please refer to \Tab{answers_statistics}.
While for \CM and \CP those are single cases, then for \CA those constitute around 10\% of all answer classes,
which makes the validation set non-representative.
For that reason we decided to merge training and validation sets, shuffle the result and  re-sample new training/validation sets with a 19:1 proportion.

After the challenge ended we performed similar analysis for the test ground-truth answers (the test set was made public after the challenge deadline).
Similarly, we found several new answer classes, constituting 10\% of test answers.
The logical explanation for this is that the challenge organizers might have assumed that the participants will pre-train their models on other, much bigger medical datasets and fine-tune them on VQA-Med.
However, considering the legal and privacy issues with medical datasets, such an approach will reward the people and teams that have access to such data.

It is also worth noting that one of the new classes introduced in the test set is \textit{ct (with gi and iv contrast)}, which in fact is the fourth variation over the same answer class mentioned before.
Considering the \textit{strict accuracy} metric, it is unclear how a system could produce the right answer given the fact that the content of the images for all those classes can be \textit{essentially the same}.

Yet another conclusion from analysis of answer distributions is that category \CA task is not well-posed.
Training a system that can generalize for this category is nearly impossible to achieve considering that:
\begin{itemize}
\item  after exclusion of \CB samples there are total 3082 training samples constituting the \CA category, and having 1483 unique answers. This means that the answer classes are extremely skewed, with median frequency of appearance of 2 and almost 37$\%$ lower than the median,
\item in majority of the cases the abnormalities are very hard to be detected and/or distinguished from normal bone, tissue and organ regions present in the images,
\item some of the answers contain \textit{errors} and do not have any logical connection with the content of the image (e.g. answer \textit{patients a and b:  acute retroperitoneal hematoma}).
\end{itemize}
%One of naive approaches here will be to train a model until it will totally overfit to the training data.


%Next: comments on BLEU - bad metric as well.

We also analyzed the ground-truth answers from the point of view of using BLEU (Bilingual Evaluation Understudy)~\cite{papineni2002bleu} as a secondary metric in the challenge.
Therefore, we calculated the number of these n-grams in the training data, shown in the \Tab{n-gram-counts}.

\begin{table}
	\begin{center}
	\begin{tabular}{ccccc}
		\toprule
		\textbf{N-gram} & \CM & \CP & \CO & \CA \\
		\midrule
		Unique Answers & 44 & 15 & 10 & 1485 \\
		\midrule
		Unigram   & 66  & 17   & 18   & 1956 \\
		Bigram    & 58  & 5    & 9    & 2804 \\
		Trigram   & 33  & 1    & 3    & 1939 \\
		Fourgram  & 9   & 0    & 0    & 1176 \\
		\bottomrule
	\end{tabular}
	\end{center}
	\caption{N-gram counts for each of the original four categories in the training set (i.e. C1 and C4 include \textit{yes} and \textit{no} answers).}
	\label{tab:n-gram-counts}
\end{table}

Please note that only answers belonging to \CM and \CA have significant number of shingles  of size greater than 2 (actually some answers in \CA also have higher order n-grams).
As the BLEU score weighs unigrams to four-grams equally (0.25 each), this metric will significantly handicap the score disregarding the correct answer.
In fact, when calculating the scores using the ground-truth answers in the validation set results in an accuracy of 1.0 and a BLEU score of 0.113.
For that reason we decided to frame the problem as a purely classification task and focus on the accuracy-related metrics, i.e. when comparing performance of our models we were collecting precision, recall and F-1 scores.


Finally, we have observed that images have different sizes, which implies that we had to resize all of them to the same size that will be accepted by our models.
After some initial trials with bigger images we decided to resize them to 224x224, which enabled straightforward transfer learning of all models pre-trained on ImageNet.
However, as we have noticed that the original size corresponds to different modalities and/or planes, we decided to use this information as an additional, third input (aside of images and questions)  to our systems.


In summary, the analysis of the dataset (distribution of questions, answers, word vocabularies, categories and image sizes) led to the following findings and the system-design related decisions:
\begin{itemize}
\item merge the original training and validation sets, shuffle and re-sample new training and validation sets in proportion 19:1,
\item use weighted random sampling during batch preparation,
\item add a fifth,  \CB category for samples with Y/N question-answer pairs,
\item focus on accuracy-related metrics rather on BLEU score,
\item avoid label (answer classes) unification and data cleaning,
\item develop a separate strategy for \CA category (and its exclusion from training of initial prototypes and input fusion modules),
\item utilize image size as additional cue/input to the system.
\end{itemize}






==> transfer_learning.tex <==
\subsection{Multi-step transfer learning}

Step 0: importing pre-trained word embeddings and image encoders:
\begin{itemize}
\item pre-trained word embeddings (GloVe, experiments with MIMIC didn't gave any improvement, due to small vocabulary of question words)
\item pre-trained image encoder (tried with simple convnets, then VGG16, then ResNet and DenseNets, at the end we used ResNet)
\end{itemize}

Step 1: pre-training question classifier:
\begin{itemize}
\item mention optimal "architecture" search - 1hot+bow, 
\item final: using LSTMs and GloVe embeddings, 
\end{itemize}

Step 2: pre-training inputs encoders:
\begin{itemize}
\item word embeddings and image encoder imported, but trainable (color: green-ish)
\item architecture search with different fusion methods (concat, EWM, MCB, CoAtt), on tasks 1,2,3 separately
\item added image size as additional modality with second fusion (concatenation)
\item finally trained the resulting "inputs encoder on 1,2,3,y/n categories" (excluding the ill-posed 4th category)
\end{itemize}

Step 3: training the final model(s):
\begin{itemize}
\item model with a single classifier: using pre-trained, trainable inputs encoders (green-ish) and classifier
\item model with 5 classifiers: using pre-trained, frozen question classifier (blue-ish) pre-trained, trainable inputs encoders (green-ish) and 5 classifiers (plus final answer fusion)
\item model with 5 classifiers and supporting facts: using pre-trained, frozen question classifier (blue-ish) pre-trained, trainable inputs encoders (green-ish), 3 supporting facts network and 5 classifiers (plus final answer fusion)
\end{itemize}

